Physically Consistent Evaluation of Commonly Used Near-Field Models

Near-field multi-antenna wireless communication has attracted growing research interest in recent years. Despite this development, most of the current literature on antennas and reflecting structures relies on simplified models, whose validity for real systems remains unclear. In this paper, we introduce a physically consistent near-field model, which we use to evaluate commonly used models. Our results indicate that common models are sufficient for basic beamfocusing, but fail to accurately predict the sidelobes and frequency dependence of reflecting structures.

==> sty/eth-colours.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% ETH Zürich's Corporate Design Colours
%%
%% Alexander Stutz (alstutz@iis.ee.ethz.ch)
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% corporate design colours
\definecolor{eth_blue}{RGB}{33, 92, 175}
\definecolor{eth_blue_10}{RGB}{233, 239, 247}
\definecolor{eth_blue_20}{RGB}{211, 222, 239}
\definecolor{eth_blue_60}{RGB}{122, 157, 207}
\definecolor{eth_blue_80}{RGB}{77, 125, 191}
\definecolor{eth_blue_120}{RGB}{8, 64, 126}

\definecolor{eth_petrol_120}{RGB}{0, 89, 109}
\definecolor{eth_petrol}{RGB}{0, 120, 148}
\definecolor{eth_petrol_10}{RGB}{231, 244, 247}
\definecolor{eth_petrol_20}{RGB}{204, 228, 234}

\definecolor{eth_green_120}{RGB}{60, 81, 30}
\definecolor{eth_green}{RGB}{98, 115, 19}
\definecolor{eth_green_10}{RGB}{239, 241, 231}
\definecolor{eth_green_20}{RGB}{224, 227, 208}
\definecolor{eth_green_60}{RGB}{161, 171, 113}
\definecolor{eth_green_80}{RGB}{129, 143, 66}
\definecolor{eth_green_120}{RGB}{54, 82, 19}

\definecolor{eth_bronze_120}{RGB}{107, 80, 31}
\definecolor{eth_bronze}{RGB}{142, 103, 19}
\definecolor{eth_bronze_10}{RGB}{244, 240, 231}

\definecolor{eth_red_120}{RGB}{150, 39, 45}
\definecolor{eth_red}{RGB}{183, 53, 45}
\definecolor{eth_red_80}{RGB}{197, 93, 87}
\definecolor{eth_red_10}{RGB}{248, 235, 234}
\definecolor{eth_red_20}{RGB}{241,215,213}

\definecolor{eth_purple_120}{RGB}{140, 10, 89}
\definecolor{eth_purple}{RGB}{167, 17, 122}
\definecolor{eth_purple_10}{RGB}{248, 232, 243}
\definecolor{eth_purple_20}{RGB}{239, 208, 227}

\definecolor{eth_grey_120}{RGB}{87, 87, 87}
\definecolor{eth_grey}{RGB}{111, 111, 111}
\definecolor{eth_grey_10}{RGB}{241, 241, 241}


% black and shades of grey
% (for non-white background check required opacity online)
\definecolor{eth_black}{RGB}{0, 0, 0}
\definecolor{eth_black_light}{RGB}{34, 34, 34}
\definecolor{eth_black_60}{RGB}{102, 102, 102}
\definecolor{eth_black_light_48}{RGB}{149,149,149}
\definecolor{eth_black_light_20}{RGB}{211, 211, 211}
\definecolor{eth_grey_10}{RGB}{241, 241, 241}
\definecolor{eth_grey_05}{RGB}{246, 246, 246}






==> sty/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Macros for the Paper 
%%
%% "Efficient and Physically-Consistent Modeling
%%  of Reconfigurable Electromagnetic Structures"
%%
%% Alexander Stutz, Georg Schwan, and Christoph Studer
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Color Palette:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sty/eth-colours}

% corporate design colors
\colorlet{blue}{eth_blue}
\colorlet{blue_10}{eth_blue_10}
\colorlet{blue_20}{eth_blue_20}
\colorlet{blue_60}{eth_blue_60}
\colorlet{blue_80}{eth_blue_80}
\colorlet{blue_120}{eth_blue_120}

\colorlet{petrol_120}{eth_petrol_120}
\colorlet{petrol}{eth_petrol}
\colorlet{petrol_10}{eth_petrol_10}
\colorlet{petrol_20}{eth_petrol_20}

\colorlet{green_120}{eth_green_120}
\colorlet{green}{eth_green}
\colorlet{green_10}{eth_green_10}
\colorlet{green_60}{eth_green_60}
\colorlet{green_80}{eth_green_80}
\colorlet{green_120}{eth_green_120}

\colorlet{bronze_120}{eth_bronze_120}
\colorlet{bronze}{eth_bronze}
\colorlet{bronze_10}{eth_bronze_10}

\colorlet{red_120}{eth_red_120}
\colorlet{red}{eth_red}
\colorlet{red_80}{eth_red_80}
\colorlet{red_10}{eth_red_10}

\colorlet{purple_120}{eth_purple_120}
\colorlet{purple}{eth_purple}
\colorlet{purple_10}{eth_purple_10}
\colorlet{purple_20}{eth_purple_20}

\colorlet{black}{eth_black}
\colorlet{black_light}{eth_black_light}
\colorlet{black_60}{eth_black_60}
\colorlet{black_light_48}{eth_black_light_48}
\colorlet{black_light_20}{eth_black_light_20}
\colorlet{grey_120}{eth_grey_120}
\colorlet{grey}{eth_grey}
\colorlet{grey_10}{eth_grey_10}
\colorlet{grey_05}{eth_grey_05}

\definecolor{pink}{RGB}{214,82,130}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tikz Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclarepatternformonly{south east lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{5pt}{5pt}}{\pgfqpoint{5pt}{5pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{5pt}}
    \pgfpathlineto{\pgfqpoint{5pt}{0pt}}
    \pgfpathmoveto{\pgfqpoint{.2pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{-.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{5.2pt}{4.8pt}}
    \pgfpathlineto{\pgfqpoint{4.8pt}{5.2pt}}
    \pgfusepath{stroke}}
    
\pgfdeclarepatternformonly{horizontal lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3.54pt}{3.54pt}}{\pgfqpoint{3.54pt}{3.54pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{2pt}}
    \pgfpathlineto{\pgfqpoint{3.54pt}{2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal behind text}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{15pt}{15pt}}{\pgfqpoint{15pt}{15pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{15pt}{15pt}}
    \pgfpathmoveto{\pgfqpoint{14.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{15.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{14.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{15.2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal pattern node}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3pt}{3pt}}{\pgfqpoint{3pt}{3pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{3pt}{3pt}}
    \pgfpathmoveto{\pgfqpoint{2.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{3.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{2.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{3.2pt}}
    \pgfusepath{stroke}}

\def\centerOfC at (#1,#2){
    \draw  [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.27,-.27) rectangle (.27,.27);
    \draw  [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.3,-.15) rectangle (.3,.15);

    
    \draw  [shift={(#1,#2)},line width=0.3pt, fill=white] (0,0) ellipse (0.16 and 0.16);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (-0.2,0) -- (0.2,0);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (0,-0.2) -- (0,0.2);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (0:0.16) arc (0:90:.16) -- cycle;
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (180:0.16) arc (180:90+180:.16) -- cycle;
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Operators:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\diag}{diag}			        % diag matrix
\DeclareMathOperator{\Ex}{\mathbb{E}}		        % expectation operator
\newcommand{\T}[0]{\mathsf{T}}                      % transpose
\newcommand{\He}[0]{\mathsf{H}}                     % hermitian
\DeclareMathOperator*{\argmax}{arg\,max}            % argmax
\DeclareMathOperator*{\maximize}{maximize}          % maximize               

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Font Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\up}[1]{{\textnormal{#1}}}              % subscripts
\newcommand{\upc}[1]{{\textnormal{\textbf{#1}}}}    % subscripts in caption

\newcommand{\mat}[1]{{\bm{\mathbf{#1}}}}            % matrices
\newcommand{\vect}[1]{{\bm{\mathbf{#1}}}}           % vectors
\newcommand{\oper}[1]{\mathbb{#1}}                  % operator

\newcommand{\phs}[1]{{\color{pink}\mathsf{#1}}}  % phasor scalar
\newcommand{\phv}[1]{{\color{pink}\bm{\mathsf{#1}}}} % phasor vector


\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Fancy Ref Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\fancyrefapplabelprefix}{app}		% Appendix
\newcommand*{\fancyrefthmlabelprefix}{thm}		% Theorem
\newcommand*{\fancyrefdefilabelprefix}{defi}    % Definition
\newcommand*{\fancyrefproplabelprefix}{prop}	% Proposition
\newcommand*{\fancyrefalglabelprefix}{alg}		% Algorithm
\newcommand*{\fancyrefasmlabelprefix}{asm}		% Assumption
\newcommand*{\fancyrefremlabelprefix}{rem}		% Remark
%\newcommand*{\fancyreftablabelprefix}{tab}		% Table


% label names
\frefformat{vario}{\fancyrefseclabelprefix}{Sec.~#1}
\frefformat{vario}{\fancyrefthmlabelprefix}{Thm.~#1}
\frefformat{vario}{\fancyrefdefilabelprefix}{Def.~#1}
\frefformat{vario}{\fancyreffiglabelprefix}{Fig.~#1}
\frefformat{vario}{\fancyrefapplabelprefix}{App.~#1}
\frefformat{vario}{\fancyrefeqlabelprefix}{(#1)}
\frefformat{vario}{\fancyrefproplabelprefix}{Prop.~#1}
\frefformat{vario}{\fancyrefalglabelprefix}{Alg.~#1}
\frefformat{vario}{\fancyrefasmlabelprefix}{Assu.~#1}
\frefformat{vario}{\fancyrefremlabelprefix}{Rem.~#1}
\frefformat{vario}{\fancyreftablabelprefix}{Table~#1}


\let\svthefootnote\thefootnote
\newcommand\blankfootnote[1]{%
  \let\thefootnote\relax\footnotetext{#1}%
  \let\thefootnote\svthefootnote%
}

%%%%% SPACE TWEAKS
\linespread{0.980625} 
\setlength{\textfloatsep}{10pt} % space under figure
\setlength{\floatsep}{10pt} % space between two figure
\setlength{\dbltextfloatsep}{10pt} % space under figure*
\setlength{\dblfloatsep}{10pt} % space between two figure*

